Image Denoising Using Global and Local Circulant Representation

The proliferation of imaging devices and countless image data generated every day impose an increasingly high demand on efficient and effective image denoising. In this paper, we establish a theoretical connection between principal component analysis (PCA) and the Haar transform under circulant representation, and present a computationally simple denoising algorithm. The proposed method, termed Haar-tSVD, exploits a unified tensor singular value decomposition (t-SVD) projection combined with Haar transform to efficiently capture global and local patch correlations. Haar-tSVD operates as a one-step, parallelizable plug-and-play denoiser that eliminates the need for learning local bases, thereby striking a balance between denoising speed and performance. Besides, an adaptive noise estimation scheme is introduced to improve robustness according to eigenvalue analysis of the circulant structure. To further enhance the performance under severe noise conditions, we integrate deep neural networks with Haar-tSVD based on the established Haar-PCA relationship. Experimental results on various denoising datasets demonstrate the efficiency and effectiveness of proposed method for noise removal. Our code is publicly available at https://github.com/ZhaomingKong/Haar-tSVD.

==> Fig_HSI_Cuprite.tex <==
\begin{figure}[htbp]
\vspace{-5.08pt}
\graphicspath{{Figs/Real_HSI_witout_ref_selected/Cuprite/Combined_new/}}
\centering
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.816in]{Cuprite_224_combined_small_new}}\hfill
\subfigure[BM4D]{
\label{Fig4}
\includegraphics[width=0.816in]{BM4D2_denoised_224_combined_small_new}}\hfill
\subfigure[RAS2S]{
\label{Fig4}
\includegraphics[width=0.816in]{RAS2S_denoised_224_combined_small_new}}\hfill
\subfigure[Haar-tSVD]{
\label{Fig4}
\includegraphics[width=0.816in]{Haar_t-SVD_denoised_224_combined_small_new}}
\vspace{-6.998pt}
\caption{Denoising comparison on the Cuprite data \cite{middleton2013earth}.}
\label{Fig_HSI_Cuprite}
\vspace{-6.8pt}
\end{figure}


==> Fig_compare_enhancement.tex <==
\begin{figure}[htbp]
\vspace{-3.68pt}
\graphicspath{{Figs/Method/Robust_Enhancement/}}
  \centering
  \includegraphics[width=3.5018in]{Fig_compare_enhancement}
  \vspace{-9.98pt}
  \caption{Comparison of denoising effects under severe noise.}
  \label{Fig_compare_enhancement}
  \vspace{-5.18pt}
\end{figure}


==> Fig_compare_with_IOCI_CANON5D.tex <==
\begin{figure}[htbp]
\vspace{-13.8pt}
\graphicspath{{Figs/Selected_color_images/IOCI/Case3/Combined_new/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.8116in]{CANON_5D_Mark4_IMG13_7_clean_combined_small_new}}
\hspace{-0.168em}%
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.8116in]{CANON_5D_Mark4_IMG13_7_noisy_combined_small_new}
\hspace{-0.168em}%
\subfigure[Condformer]{
\label{Fig4}
\includegraphics[width=0.8116in]{CANON_5D_Mark4_IMG13_7_noisy_Condformer_combined_small_new}}
\hspace{-0.168em}%
\subfigure[DeepSN]{
\label{Fig4}
\includegraphics[width=0.8116in]{CANON_5D_Mark4_IMG13_7_noisy_DeepSN_combined_small_new}}
\hspace{-0.168em}%
\vspace{-3.18pt}
\subfigure[DIDN]{
\label{Fig4}
\includegraphics[width=0.8116in]{CANON_5D_Mark4_IMG13_7_noisy_DIDN_combined_small_new}}
\hspace{-0.168em}%
\subfigure[NAFNet]{
\label{Fig4}
\includegraphics[width=0.8116in]{CANON_5D_Mark4_IMG13_7_noisy_CBDNet_combined_small_new}}
\hspace{-0.168em}%
\subfigure[Restormer]{
\label{Fig4}
\includegraphics[width=0.8116in]{CANON_5D_Mark4_IMG13_7_noisy_Restormer_combined_small_new}}
\hspace{-0.168em}%
\subfigure[A-Haar-tSVD]{
\label{Fig4}
\includegraphics[width=0.8116in]{A_Haar_tSVDCANON_5D_Mark4_IMG13_7_noisy_combined_small_new}}
\vspace{-3.8pt}
\caption{Denoising results of compared methods on the IOCI datset.}
\label{Fig_compare_with_IOCI_CANON5D}
\vspace{0pt}
\end{figure}


==> Fig_compare_with_IOCI_CANON5D_new.tex <==
\begin{figure}[htbp]
\vspace{-6.8pt}
\graphicspath{{Figs/Selected_color_images/IOCI/Case1_new/Combined/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.80016in]{CANON_5D_Mark4_IMG13_2_clean_combined_small_new}}
\hspace{-0.168em}%
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.80016in]{CANON_5D_Mark4_IMG13_2_noisy_combined_small_new}}
\hspace{-0.168em}%
\subfigure[Condformer]{
\label{Fig4}
\includegraphics[width=0.80016in]{CANON_5D_Mark4_IMG13_2_noisy_Condformer_combined_small_new}}
\hspace{-0.168em}%
\subfigure[DeepSN]{
\label{Fig4}
\includegraphics[width=0.80016in]{CANON_5D_Mark4_IMG13_2_noisy_DeepSN_combined_small_new}}
\hspace{-0.168em}%
\vspace{-3.18pt}
\subfigure[MaIR]{
\label{Fig4}
\includegraphics[width=0.80016in]{CANON_5D_Mark4_IMG13_2_noisy_MaIR_combined_small_new}}
\hspace{-0.168em}%
\subfigure[Noise2VST]{
\label{Fig4}
\includegraphics[width=0.80016in]{CANON_5D_Mark4_IMG13_2_noisy_Noise2VST_combined_small_new}}
\hspace{-0.168em}%
\subfigure[Restormer]{
\label{Fig4}
\includegraphics[width=0.80016in]{CANON_5D_Mark4_IMG13_2_noisy_Restormer_combined_small_new}}
\hspace{-0.168em}%
\subfigure[A-Haar-tSVD]{
\label{Fig4}
\includegraphics[width=0.80016in]{A_Haar_tSVDCANON_5D_Mark4_IMG13_2_noisy_combined_small_new}}
\vspace{-6.18pt}
\caption{Denoising results of compared methods on the IOCI datset.}
\label{Fig_compare_with_IOCI_CANON5D_new}
\vspace{1.28pt}
\end{figure}


==> Fig_compare_with_IOCI_FUJI.tex <==
\begin{figure}[htbp]
\vspace{-9.8pt}
\graphicspath{{Figs/Selected_color_images/IOCI/Case5/Combined/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.8116in]{Fuji_X100T_IMG10_2_clean_combined_marked}} \hfill
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.8116in]{Fuji_X100T_IMG10_2_noisy_combined_marked}}\hfill
\subfigure[Condformer]{
\label{Fig4}
\includegraphics[width=0.8116in]{Fuji_X100T_IMG10_2_noisy_Condformer_combined_marked}}\hfill
\subfigure[DeepSN]{
\label{Fig4}
\includegraphics[width=0.8116in]{Fuji_X100T_IMG10_2_noisy_DeepSN_combined_marked}}\hfill
\vspace{-6.8pt}
\subfigure[DIDN]{
\label{Fig4}
\includegraphics[width=0.8116in]{Fuji_X100T_IMG10_2_noisy_DIDN_combined_marked}}\hfill
\subfigure[NAFNet]{
\label{Fig4}
\includegraphics[width=0.8116in]{Fuji_X100T_IMG10_2_noisy_NAFNet_combined_marked}}\hfill
\subfigure[Restormer]{
\label{Fig4}
\includegraphics[width=0.8116in]{Fuji_X100T_IMG10_2_noisy_Restormer_combined_marked}}\hfill
\subfigure[A-Haar-tSVD]{
\label{Fig4}
\includegraphics[width=0.8116in]{Haar-tSVD_hand_tune_10_2_combined_marked}}
\vspace{-2.8pt}
\caption{Denoising results of compared methods on the IOCI datset.}
\label{Fig_compare_with_IOCI_FUJI}
\end{figure}


==> Fig_compare_with_Real_HSI_case5.tex <==
\begin{figure}[htbp]
\vspace{-6.98pt}
\graphicspath{{Figs/Selected_color_images/Real-HSI/Case5/Combined/}}
\centering
%\subfigure[Noisy]{
%\label{Fig4}
%\includegraphics[width=0.816in]{noisy_53_slice_19_combined_marked}}\hfill
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=0.816in]{clean_53_slice_19_combined_marked}}\hfill
\subfigure[LTDL]{
\label{Fig4}
\includegraphics[width=0.816in]{im_denoised_LTDL_53_slice_19_combined_marked}}\hfill
\subfigure[RAS2S]{
\label{Fig4}
\includegraphics[width=0.816in]{im_denoised_RAS2S_53_slice_19_combined_marked}}\hfill
\subfigure[A-Haar-tSVD]{
\label{Fig4}
\includegraphics[width=0.816in]{im_denoised_Haar_tSVD_53_slice_19_combined_marked}}
\vspace{-6.98pt}
\caption{Denoising comparison on the Real-HSI dataset.}
\vspace{-2.8pt}
\label{Fig_compare_with_Real_HSI_case5}
\end{figure}



==> Fig_illus_dataset.tex <==
%\begin{figure}[htbp]
%\vspace{-1.8pt}
%\graphicspath{{Figs/Fig_dataset_illus/}}
%  \centering
%  \includegraphics[width=3.26in]{Fig_illus_dataset}
%   \vspace{-1.9pt}
%  \caption{Illustrations of popular denoising datasets.}
%  \label{Fig_illus_dataset}
%  \vspace{-0.6pt}
%\end{figure}
%\begin{figure}[htbp]
%\vspace{-3.8pt}
%\graphicspath{{Figs/Selected_color_images/Kodak_selected/sigma_40_30_50/Combined/}}
%\centering
%\subfigure[Noise-free]{
%\label{Fig4}
%\includegraphics[width=0.788in]{Clean_23_combined}} \hfill
%\hspace{-0.2pt}
%\subfigure[Noisy]{
%\label{Fig4}
%\includegraphics[width=0.788in]{Noisy_23_combined}} \hfill
%\subfigure[FFDNet]{
%\label{Fig4}
%\includegraphics[width=0.788in]{FFDNet_kodak_23_combined}} \hfill
%\subfigure[MaIR]{
%\label{Fig4}
%\includegraphics[width=0.788in]{kodim23_MaIR_combined}} \hfill
%\subfigure[Noise2VST]{
%\label{Fig4} 
%\includegraphics[width=0.788in]{kodim23_Noise2VST_combined}} \hfill
%\subfigure[Restormer]{
%\label{Fig4}
%\includegraphics[width=0.788in]{kodim23_Restormer_combined}} \hfill
%\subfigure[CBM3D]{
%\label{Fig4}
%\includegraphics[width=0.788in]{BM3D_kodak_23_combined}} \hfill
%\subfigure[A-Haar-tSVD]{
%\label{Fig4}
%\includegraphics[width=0.788in]{GCP_A_Haar_kodak_23_combined}} \hfill
%\vspace{-2.8pt}
%\caption{Influence of real-world noise on patch-search and rank position $a$.}
%\vspace{-3.8pt}
%\label{Fig_Kodak_high_noise}
%\end{figure} 
%%%%%%%%%%@###########################
\begin{figure}[htbp]
\vspace{-3.8pt}
\graphicspath{{Figs/Fig_dataset_illus/}}
\centering
\subfigure[Image]{%
  \includegraphics[width=0.80116in]{Color_image}}%
\hspace{0.368em}%
\subfigure[Video]{%
  \includegraphics[width=0.80116in]{Color_video}}%
\hspace{0.368em}%
\subfigure[HSI]{%
  \includegraphics[width=0.80116in]{MSI}}%
\hspace{0.368em}%
\subfigure[MRI]{%
  \includegraphics[width=0.80116in]{MRI}}%
\vspace{-0.8pt}
\caption{Popular image denoising datasets and their self-similarity.}
\vspace{-5.8pt}
\label{Fig_illus_dataset}
\end{figure}
%%%###################################$$$
%\begin{figure}[htbp]
%\vspace{-3.8pt}
%\graphicspath{{Figs/Fig_dataset_illus/}}
%\centering
%\subfigure[Image]{%
%  \includegraphics[width=0.80116in]{Color_Image_new}}%
%\hspace{0.368em}%
%\subfigure[Video]{%
%  \includegraphics[width=0.80116in]{Video_new}}%
%\hspace{0.368em}%
%\subfigure[HSI]{%
%  \includegraphics[width=0.80116in]{MSI_new2}}%
%\hspace{0.368em}%
%\subfigure[MRI]{%
%  \includegraphics[width=0.80116in]{MRI_3D_visualize}}%
%\vspace{-0.8pt}
%\caption{Illustration of popular image denoising datasets and their intrinsic self-similarity properties.}
%\vspace{-5.8pt}
%\label{Fig_illus_dataset}
%\end{figure}


==> Fig_robust_enhance_comparison_DND.tex <==
\begin{figure}[htbp]
\vspace{-2.8pt}
\graphicspath{{Figs/Method/Robust_Enhancement/DND/combined/}}
\centering
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.83018in]{Noisy_img_1_9_est_sigma_29_combined}}
\hspace{-0.398em}%
\subfigure[CBM3D]{
\label{Fig4}
\includegraphics[width=0.83018in]{CBM3D2_img_1_9_sigma_87_combined}}
\hspace{-0.398em}%
\subfigure[A-Haar-tSVD]{
\label{Fig4}
\includegraphics[width=0.83018in]{GCP_Haar_epoch_89_1_9_sigma_104_combined}}
\hspace{-0.398em}%
\subfigure[RA-Haar-tSVD]{
\label{Fig4}
\includegraphics[width=0.83018in]{GCP_CID_FCN_1_9_estsigma_104_combined}}
\vspace{-5.18pt}
\caption{Denoising effects of the robust enhancement strategy on DND.}
\label{Fig_robust_enhance_comparison_DND}
\vspace{-6.8pt}
\end{figure} 

==> Table_compare_Haar_tSVD_w_wo_GCP.tex <==
% Table generated by Excel2LaTeX from sheet 'Haar_tSVD_W_WO_GCP'
\begin{table}[htbp]
\scriptsize
  \centering
  \caption{Haar-tSVD w/wo the GCP-based patch search strategy.}
    \begin{tabular}{ccccc}
    \toprule
    Implementation & CC15  & HighISO & SIDD-val & Time (s) \\
    \midrule
    Without GCP & 37.87/0.959 & 40.45/0.973 & 34.69/0.873 & 3.6 \\
    \midrule
    With GCP & \textbf{38.10/0.961} & \textbf{40.51/0.973} & \textbf{34.78/0.880} & \textbf{3.1} \\
    \bottomrule
    \end{tabular}%
  \label{Table_compare_Haar_tSVD_w_wo_GCP}%
\end{table}%


==> Table_dataset_info_full.tex <==
%\begin{table}[htbp]
%\tiny
%  \centering
%  \caption{Popular datasets for synthetic and real-world experiments. 'GT': ground-truth, '$\surd$': Available, '-': Not available.}
%  \vspace{-3.8pt}
%  \renewcommand{\arraystretch}{0.998}
%  \scalebox{0.9699}{
%    \begin{tabular}{cccccc}
%    \toprule
%    Applications & Name  & Experiments & GT    & Image size & \# Images \\
%    \midrule
%    \multicolumn{1}{c}{\multirow{6}[16]{*}{Image}} & Kodak \cite{Kodak} & Synthetic & $\surd$     & 512 $\times$ 512 $\times$ 3 & 24 \\
%%\cmidrule{2-6}          & RENOIR \cite{anaya2018renoir} & Real-world & $\surd$     & 3684 $\times$ 2760 $\times$ 3 & 120 \\
%\cmidrule{2-6}          & Nam-CC \cite{nam2016holistic} & Real-world & $\surd$     & 512 $\times$ 512 $\times$ 3 & 15 \\
%\cmidrule{2-6}          & PolyU \cite{xu2018real} & Real-world & $\surd$     & 512 $\times$ 512 $\times$ 3 & 100 \\
%\cmidrule{2-6}          & DnD \cite{plotz2017benchmarking} & Real-world & -   & 512 $\times$ 512 $\times$ 3 & 1000 \\
%\cmidrule{2-6}          & SIDD \cite{abdelhamed2018high} & Real-world & -   & 256 $\times$ 256 $\times$ 3 & 1280 \\
%\cmidrule{2-6}          & HighISO \cite{yue2019high} & Real-world & $\surd$     & 512 $\times$ 512 $\times$ 3 & 100 \\
%\cmidrule{2-6}          & IOCI \cite{kong2023comparison} & Real-world & $\surd$     & 1024 $\times$ 1024 $\times$ 3 & 848 \\
%    \midrule
%    \multirow{3}[6]{*}{Video} & Set8 \cite{Set8} & Synthetic & $\surd$     & 960 $\times$ 540 $\times$ 3 $\times$ frames & 8 \\
%\cmidrule{2-6}          & CRVD \cite{yue2020supervised} & Real-world & $\surd$     & 1920 $\times$ 1080 $\times$ 3 $\times$ frames & 55 \\
%\cmidrule{2-6}          & IOCV \cite{kong2023comparison} & Real-world & $\surd$     & 512 $\times$ 512 $\times$ 3 $\times$ frames & 39 \\
%    \midrule
%    \multirow{5}[5]{*}{MSI/HSI} & Real-HSI \cite{zhang2021hyperspectral} & Real-world & $\surd$     & 696 $\times$ 520 $\times$ 34 & 59 \\
%\cmidrule{2-6}          & ICVL \cite{arad_and_ben_shahar_2016} & Synthetic & $\surd$     & 1392 $\times$ 1300 $\times$ 31 & 201 \\
%%\cmidrule{2-6}          & Indian Pines \cite{PURR1947} & Synthetic & $\surd$     & 145 $\times$ 145 $\times$ 224 & 1 \\
%\cmidrule{2-6}          & Urban \cite{PURR1947} & Real-world & -   & 307 $\times$ 307 $\times$ 210 & 1 \\
%\cmidrule{2-6}          & HHD \cite{chakrabarti2011statistics} & Real-world & -   & 1392 $\times$ 1040 $\times$ 31 & 77 \\    \bottomrule
%    \end{tabular}%
%    }
%  \label{Table_dataset_description}%
%\end{table}% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
\tiny
  \centering
  \caption{Popular datasets for synthetic and real-world experiments. `GT': ground-truth, `\Checkmark': Available, `-': Not available.}
  \vspace{-3.98pt}
  \renewcommand{\arraystretch}{0.9998}
  \scalebox{0.9618}{
    \begin{tabular}{cccccc}
    \toprule
    Applications & Name  & Experiments & GT    & Image size & \# Images \\
    \midrule
    \multicolumn{1}{c}{\multirow{6}[12]{*}{Image}} & Kodak \cite{Kodak} & Synthetic & \Checkmark     & 512 $\times$ 512 $\times$ 3 & 24 \\
%\cmidrule{2-6}          & RENOIR \cite{anaya2018renoir} & Real-world & \Checkmark     & 3684 $\times$ 2760 $\times$ 3 & 120 \\
\cmidrule{2-6}          & Nam-CC \cite{nam2016holistic} & Real-world & \Checkmark     & 512 $\times$ 512 $\times$ 3 & 15 \\
\cmidrule{2-6}          & PolyU \cite{xu2018real} & Real-world & \Checkmark     & 512 $\times$ 512 $\times$ 3 & 100 \\
\cmidrule{2-6}          & DnD \cite{plotz2017benchmarking} & Real-world & -   & 512 $\times$ 512 $\times$ 3 & 1000 \\
\cmidrule{2-6}          & SIDD \cite{abdelhamed2018high} & Real-world & -   & 256 $\times$ 256 $\times$ 3 & 1280 \\
\cmidrule{2-6}          & HighISO \cite{yue2019high} & Real-world & \Checkmark     & 512 $\times$ 512 $\times$ 3 & 100 \\
\cmidrule{2-6}          & IOCI \cite{kong2023comparison} & Real-world & \Checkmark     & 1024 $\times$ 1024 $\times$ 3 & 848 \\
    \midrule
    \multirow{2}[1]{*}{Video} & CRVD \cite{yue2020supervised} & Real-world & \Checkmark     & 1920 $\times$ 1080 $\times$ 3 $\times$ frames & 55 \\
\cmidrule{2-6}          & IOCV \cite{kong2023comparison} & Real-world & \Checkmark     & 512 $\times$ 512 $\times$ 3 $\times$ frames & 39 \\
    \midrule
    \multirow{5}[5]{*}{HSI} & Real-HSI \cite{zhang2021hyperspectral} & Real-world & \Checkmark     & 696 $\times$ 520 $\times$ 34 & 59 \\
\cmidrule{2-6}          & ICVL \cite{arad_and_ben_shahar_2016} & Synthetic & \Checkmark     & 1392 $\times$ 1300 $\times$ 31 & 201 \\
%\cmidrule{2-6}          & Indian Pines \cite{PURR1947} & Synthetic & \Checkmark     & 145 $\times$ 145 $\times$ 224 & 1 \\
\cmidrule{2-6}          & Urban \cite{PURR1947} & Real-world & -   & 307 $\times$ 307 $\times$ 210 & 1 \\
\cmidrule{2-6}          & HHD \cite{chakrabarti2011statistics} & Real-world & -   & 1392 $\times$ 1040 $\times$ 31 & 77 \\    \bottomrule
    \end{tabular}%
    }
  \label{Table_dataset_description}%
\end{table}% 
